A Static Analysis of Informed Down-Samples

We present an analysis of the loss of population-level test coverage induced by different down-sampling strategies when combined with lexicase selection. We study recorded populations from the first generation of genetic programming runs, as well as entirely synthetic populations. Our findings verify the hypothesis that informed down-sampling better maintains population-level test coverage when compared to random down-sampling. Additionally, we show that both forms of down-sampling cause greater test coverage loss than standard lexicase selection with no down-sampling. However, given more information about the population, we found that informed down-sampling can further reduce its test coverage loss. We also recommend wider adoption of the static population analyses we present in this work.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.79.  Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.80.  New journals: DLT, FAC


==> scratch.tex <==
==== 2023-02-09 Original background / methods ====

\section{Background}
\todo{Ryan}{Replace paragraphs with one line each}
%\paragraph{Lexicase Selection}

%Lexicase selection \citep{assessment_spector_2012, Helmuth_solving_2015} is a parent selection algorithm that does not aggregate performance or error metrics for use in selection. Instead, with the cases shuffled into a random order, the population is filtered down to maintain solely the individuals that are elite (best in the population) on each test case, in the order that they are seen. This process is halted if there are no test cases left, upon which a random individual is chosen from the remaining ones, or if a single individual remains in the candidate pool, upon which this individual is selected. After each selection event, the cases are shuffled and the process repeats from the beginning for the next selection event.

%\paragraph{Down-sampled Lexicase Selection}
 %First proposed for expensive evolutionary robotics runs, down-sampled lexicase selection \cite{moore2017lex} is the process of not using the entire training set for each selection event, but instead restricting all selection events in a single generation to use the same smaller set of training cases. Random down-sampled lexicase selection was later formalized by \citet{hernandez_random_2019} and studied by \citet{Helmuth2021benefits} for its use in genetic programming runs. Instead of being used to reduce computational needs, runs using down-sampling were run for many more generations such that the total number of program executions is the same as those in standard lexicase selection. This resulted in significant improvements in problem solving performance over standard lexicase selection. \citet{helmuth_explaining_2020} perform experiments to determine that this added benefit is simply due to more individuals being explored, although each less thoroughly. Various studies have since been performed to explore \cite{ferguson_characterizing_2020, moore_objective_2021, boldi_2022_environmental, helmuth_applying_2022} or build upon \cite{boldi_informed_2023} these results.

 \paragraph{Informed Down-sampled Lexicase Selection}
In order to help solve some hypothesized issues with random down-sampling, informed down-sampled lexicase selection \cite{boldi_informed_2023} was proposed. Informed down-sampling was designed to limit the number of important cases that are not used for selection each generation. It works by defining the distance between two cases as the differences in the distributions of individuals that solve them. For example, two cases that are solved by the same group of individuals have zero distance and are thus synonymous, and two cases that are solved by complementary groups of individuals have a high distance and are thus mutually informative. Informed down-sampling was verified to indeed significantly improve the problem solving performance of genetic programming systems when performing program synthesis. 

In this work, we explore informed down-sampling based on full information and sparse information. Full information informed down-sampling is where the entire population is evaluated on the entire training set in order to select a down-sample that is informative with respect to the entire current population. This process is counter intuitive as we are evaluating on all training cases, and could just use these evaluations for selection instead of bothering with down-sampling. Despite this, this process shows us what we could expect if we did have all the information we needed about the current population. As a noisy version of this, that does not require full information about the population, is sparse information informed down-sampling (IDS). Instead of using the whole population, IDS considers a set of parent representatives (usually 1\% of all the individuals) that are used to evaluate the distances between cases. For a more in depth discussion of informed down-sampling, please see the work by \citet{boldi_informed_2023}.
 

\paragraph{Test Coverage} Every population contains individuals that solve various subsets of the training set. The test coverage of a population is the number of training cases that have at least one individual that solves them. This value helps measure how the population's performance across the training set changes over evolutionary time. Test coverage is an important metric to measure problem solving progress. It gives a signal regarding the number of test cases this population currently has knowledge\footnote{Knowledge here could constitute some genetic material that encodes a portion of the desired problem solution.} about. A loss of test coverage could be counter-productive for evolutionary search, as important building blocks to the final solution are being lost from the population.


\section{Methods}
\todo{Alex}{weave in your synthetic stuff}
Our investigation involves analyzing real populations that were extracted from the first generation of program synthesis evolutionary runs. 40 random populations configured to solve the Count Odds problem, and 40 more configured to solve the Fizz Buzz problem were analyzed in the following way.

We measure the test case coverage for each population before any selection is performed. This is the maximum possible test case coverage achievable by any selection event as there is no mutation or further evolution. Then, we perform lexicase selection ten times on this population for each of four different down-sampling strategies and three different down-sample rates. The strategies that we study here are using a full information informed down-sample, a sparse information informed down-sample, a random down-sample and no down-sampling (standard lexicase). We perform all down-sampling at three different levels: 0.05, 0.1 and 0.2, meaning 5\%, 10\% or 20\% of the entire training set is included in each of the down-samples. Each of these selections results in a population of the same size as we started with. Then, we measure the test coverage for each of these populations. To compare against the baseline, we compute and record the test case coverage \emph{loss} that occurred during each of these selection events.


===============

% reduced test case coverage than  between generations and that informed down-sampling is helping by remedying this issue. First, we investigate randomly generated populations that could be evolved to solve the count odds and fizz buzz program synthesis problems. Then, we extend this investigation to a set of synthetic populations.

% We measure the test coverage before and after selection for a set of real and synthetic genetic programming populations. We compare the effect on test coverage that each of three down-sampling methods have. We compare lexicase selection as a baseline with no down-sampling with full information informed down-sampling, sparse information informed down-sampling and random down-sampling. Through these experiments, we find that random down-sampling does indeed result in significant test coverage loss, while standard lexicase would loses little to no test coverage. Informed down-sampling with sparse information remedies this slightly, and informed down-sampling with full information remedies it nearly entirely.

% \section{Background}
% \todo{Ryan}{Replace paragraphs with one line each}
%\paragraph{Lexicase Selection}

%Lexicase selection \citep{assessment_spector_2012, Helmuth_solving_2015} is a parent selection algorithm that does not aggregate performance or error metrics for use in selection. Instead, with the cases shuffled into a random order, the population is filtered down to maintain solely the individuals that are elite (best in the population) on each test case, in the order that they are seen. This process is halted if there are no test cases left, upon which a random individual is chosen from the remaining ones, or if a single individual remains in the candidate pool, upon which this individual is selected. After each selection event, the cases are shuffled and the process repeats from the beginning for the next selection event.

%\paragraph{Down-sampled Lexicase Selection}
 %First proposed for expensive evolutionary robotics runs, down-sampled lexicase selection \cite{moore2017lex} is the process of not using the entire training set for each selection event, but instead restricting all selection events in a single generation to use the same smaller set of training cases. Random down-sampled lexicase selection was later formalized by \citet{hernandez_random_2019} and studied by \citet{Helmuth2021benefits} for its use in genetic programming runs. Instead of being used to reduce computational needs, runs using down-sampling were run for many more generations such that the total number of program executions is the same as those in standard lexicase selection. This resulted in significant improvements in problem solving performance over standard lexicase selection. \citet{helmuth_explaining_2020} perform experiments to determine that this added benefit is simply due to more individuals being explored, although each less thoroughly. Various studies have since been performed to explore \cite{ferguson_characterizing_2020, moore_objective_2021, boldi_2022_environmental, helmuth_applying_2022} or build upon \cite{boldi_informed_2023} these results.

 % \paragraph{Informed Down-sampled Lexicase Selection}
% In order to help solve some hypothesized issues with random down-sampling, informed down-sampled lexicase selection \cite{boldi_informed_2023} was proposed. Informed down-sampling was designed to limit the number of important cases that are not used for selection each generation. It works by defining the distance between two cases as the differences in the distributions of individuals that solve them. For example, two cases that are solved by the same group of individuals have zero distance and are thus synonymous, and two cases that are solved by complementary groups of individuals have a high distance and are thus mutually informative. Informed down-sampling was verified to indeed significantly improve the problem solving performance of genetic programming systems when performing program synthesis. 

% In this work, we explore informed down-sampling based on full information and sparse information. Full information informed down-sampling is where the entire population is evaluated on the entire training set in order to select a down-sample that is informative with respect to the entire current population. This process is counter intuitive as we are evaluating on all training cases, and could just use these evaluations for selection instead of bothering with down-sampling. Despite this, this process shows us what we could expect if we did have all the information we needed about the current population. As a noisy version of this, that does not require full information about the population, is sparse information informed down-sampling (IDS). Instead of using the whole population, IDS considers a set of parent representatives (usually 1\% of all the individuals) that are used to evaluate the distances between cases. For a more in depth discussion of informed down-sampling, please see the work by \citet{boldi_informed_2023}.
 

% \paragraph{Test Coverage} Every population contains individuals that solve various subsets of the training set. The test coverage of a population is the number of training cases that have at least one individual that solves them. This value helps measure how the population's performance across the training set changes over evolutionary time. Test coverage is an important metric to measure problem solving progress. It gives a signal regarding the number of test cases this population currently has knowledge\footnote{Knowledge here could constitute some genetic material that encodes a portion of the desired problem solution.} about. A loss of test coverage could be counter-productive for evolutionary search, as important building blocks to the final solution are being lost from the population.

% In order to help solve some hypothesized issues with random down-sampling, informed down-sampled lexicase selection \cite{boldi_informed_2023} was proposed. Informed down-sampling was designed to limit the number of important cases that are not used for selection each generation. It works by defining the distance between two cases as the differences in the distributions of individuals that solve them. For example, two cases that are solved by the same group of individuals have zero distance and are thus synonymous, and two cases that are solved by complementary groups of individuals have a high distance and are thus mutually informative. Informed down-sampling was verified to indeed significantly improve the problem solving performance of genetic programming systems when performing program synthesis. 


% In this work, we explore informed down-sampling based on full information and sparse information. Full information informed down-sampling is where the entire population is evaluated on the entire training set in order to select a down-sample that is informative with respect to the entire current population. This process is counter intuitive as we are evaluating on all training cases, and could just use these evaluations for selection instead of bothering with down-sampling. Despite this, this process shows us what we could expect if we did have all the information we needed about the current population. As a noisy version of this, that does not require full information about the population, is sparse information informed down-sampling (IDS). Instead of using the whole population, IDS considers a set of parent representatives (usually 1\% of all the individuals) that are used to evaluate the distances between cases. For a more in depth discussion of informed down-sampling, please see the work by \citet{boldi_informed_2023}.

% Every population contains individuals that solve various subsets of the training set. The test coverage of a population is the number of training cases that have at least one individual that solves them. This value helps measure how the population's performance across the training set changes over evolutionary time. Test coverage is an important metric to measure problem solving progress. It gives a signal regarding the number of test cases this population currently has knowledge\footnote{Knowledge here could constitute some genetic material that encodes a portion of the desired problem solution.} about. A loss of test coverage could be counter-productive for evolutionary search, as important building blocks to the final solution are being lost from the population.

% We measure the test case coverage for each population before any selection is performed. This is the maximum possible test case coverage achievable by any selection event as there is no mutation or further evolution. Then, we perform lexicase selection ten times on this population for each of four different down-sampling strategies and three different down-sample rates. The strategies that we study here are using a full information informed down-sample, a sparse information informed down-sample, a random down-sample and no down-sampling (standard lexicase). We perform all down-sampling at three different levels: 0.05, 0.1 and 0.2, meaning 5\%, 10\% or 20\% of the entire training set is included in each of the down-samples. Each of these selections results in a population of the same size as we started with. Then, we measure the test coverage for each of these populations. To compare against the baseline, we compute and record the test case coverage \emph{loss} that occurred during each of these selection events.
